A dusty proto-cluster surrounding the binary galaxy HerBS-70 at $z = 2.3$

We report on deep SCUBA-2 observations at 850$\mu$m and NOEMA spectroscopic measurements at 2 mm of the environment surrounding the luminous, massive ($M_{*} \approx 2 \times 10^{11}$ M$_{\odot}$) Herschel-selected source HerBS-70. This source was revealed by previous NOEMA observations to be a binary system of dusty star-forming galaxies at $z= 2.3$, with the East component (HerBS-70E) hosting an Active Galactic Nucleus (AGN). The SCUBA-2 observations detected, in addition to the binary system, twenty-one sources at $> 3.5 \sigma$ over an area of $\sim 25$ square comoving Mpc with a sensitivity of $\sigma_{850} = 0.75$ mJy. The surface density of continuum sources around HerBS-70 is three times higher than for field galaxies. The NOEMA spectroscopic measurements confirm the protocluster membership of three of the nine brightest sources through their CO(4 - 3) line emission, yielding a volume density 36 times higher than for field galaxies. All five confirmed sub-mm galaxies in the HerBS-70 system have relatively short gas depletion times ($80 - 500$ Myr), indicating the onset of quenching for this protocluster core due to the depletion of gas. The dark matter halo mass of the HerBS-70 system is estimated around $5 \times{} 10^{13}$ M$_{\odot}$, with a projected current-day mass of $10^{15}$ M$_{\odot}$, similar to the local Virgo and Coma clusters. These observations support the claim that DSFGs, in particular the ones with observed multiplicity, can trace cosmic overdensities.

==> table_with_sourcefluxes.tex <==

%Table of sources
% \begin{landscape}
{ 
% \resizebox{\textwidth}{!}{
% \hspace{-3cm}
% \onecolumn
% \begin{adjustbox}{angle=90}
\begin{table*}
    \caption{Observed and derived properties of sources detected at 850\micron{} in the field surrounding HerBS-70}
    \label{tab:sources}
    % \centering
    \begin{tabular}{rccrcccccccccc} \hline
\# & RA & DEC & SNR & $z_{\rm phot}$  & SFR & $L_{\rm FIR}$ & $M_{\rm dust}$ & $S_{\rm 250 \mu m}$& $S_{\rm 350 \mu m}$& $S_{\rm 500 \mu m}$& $S_{\rm 850 \mu m}$' & Bias & $\mathcal{F}$ \\ 
& [hms] & [dms] & & & [M$_{\odot}$/yr]& [$10^{12} L_{\odot}$]& [$10^9 M_{\odot}$] & [mJy]& [mJy]& [mJy]& [mJy] \\
\hline
70EW  & 13:01:40.3 & +29:29:16 & 22.6 & 1.8 $\pm$ 0.4 & 1800 & 10.2 & 5.3 & 122.3 $\pm$ 6.1 & 139.3 $\pm$ 5.6 & 106.4 $\pm$ 6.0 & 16.9 $\pm$ 1.9 & 1.00 & 0.0\\
70.S1 & 13:01:35.4 & +29:28:00 & 8.9 & 3.4 $\pm$ 0.6 & 780 & 4.6 & 2.4 & 11.9 $\pm$ 6.1$^{\dagger}$ & 12.6 $\pm$ 5.6$^{\dagger}$ & 15.7 $\pm$ 6.0$^{\dagger}$ & 7.5 $\pm$ 1.2 & 1.00 & 0.0\\
70.S2 & 13:01:44.0 & +29:29:04 & 6.8 & 2.0 $\pm$ 0.4 & 550 & 3.2 & 1.7 & 23.3 $\pm$ 6.1$^{\dagger}$ & 32.4 $\pm$ 5.6$^{\dagger}$ & 28.7 $\pm$ 6.0$^{\dagger}$ & 5.3 $\pm$ 1.1 & 1.01 & 0.0\\
70.S3 & 13:02:00.3 & +29:27:24 & 6.6 & 1.7 $\pm$ 0.4 & 750 & 4.4 & 2.3 & 54.0 $\pm$ 6.0 & 57.5 $\pm$ 5.5 & 40.3 $\pm$ 6.3 & 7.2 $\pm$ 1.5 & 1.01 & 0.0\\
70.S4 & 13:01:46.7 & +29:29:28 & 6.5 & 1.7 $\pm$ 0.4 & 580 & 3.4 & 1.8 & 34.2 $\pm$ 6.1 & 37.4 $\pm$ 5.6 & 20.6 $\pm$ 6.1 & 5.6 $\pm$ 1.2 & 1.01 & 0.0\\
70.S5 & 13:01:18.0 & +29:28:08 & 5.1 & 2.6 $\pm$ 0.5 & 670 & 3.9 & 2.0 & 16.3 $\pm$ 6.1$^{\dagger}$ & 19.5 $\pm$ 5.6$^{\dagger}$ & 12.8 $\pm$ 6.0$^{\dagger}$ & 6.5 $\pm$ 1.8 & 1.01 & 0.0\\
70.S6 & 13:01:44.3 & +29:30:28 & 5.0 & 2.0 $\pm$ 0.4 & 430 & 2.5 & 1.3 & 17.9 $\pm$ 6.0 & 19.8 $\pm$ 5.3 & 6.5 $\pm$ 6.3 & 4.2 $\pm$ 1.2 & 1.01 & 0.0\\
70.S7 & 13:01:56.9 & +29:31:08 & 4.7 & 3.5 $\pm$ 0.6 & 540 & 3.1 & 1.6 & 6.2 $\pm$ 6.1$^{\dagger}$ & 9.5 $\pm$ 5.6$^{\dagger}$ & 12.5 $\pm$ 6.0$^{\dagger}$ & 5.2 $\pm$ 1.6 & 1.01 & 0.0\\
70.S8 & 13:01:33.3 & +29:29:28 & 4.3 & 2.8 $\pm$ 0.5 & 400 & 2.3 & 1.2 & 6.1 $\pm$ 6.1$^{\dagger}$ & 13.2 $\pm$ 5.6$^{\dagger}$ & 6.1 $\pm$ 6.0$^{\dagger}$ & 3.9 $\pm$ 1.2 & 1.02 & 0.0\\
70.S9 & 13:02:00.0 & +29:30:16 & 4.3 & 1.3 $\pm$ 0.3 & 520 & 3.0 & 1.6 & 58.4 $\pm$ 5.9 & 46.2 $\pm$ 5.9 & 25.8 $\pm$ 6.5 & 5.0 $\pm$ 1.6 & 1.02 & 0.0\\
70.S10 & 13:01:27.8 & +29:23:40 & 4.2 & 3.6 $\pm$ 0.6 & 1100 & 6.6 & 3.4 & 13.1 $\pm$ 6.1$^{\dagger}$ & 19.0 $\pm$ 5.6$^{\dagger}$ & 16.7 $\pm$ 6.0$^{\dagger}$ & 10.9 $\pm$ 3.5 & 1.02 & 0.0\\
70.S11 & 13:01:22.0 & +29:30:24 & 4.1 & 0.7 $\pm$ 0.2 & 460 & 2.7 & 1.4 & 102.5 $\pm$ 6.0 & 57.1 $\pm$ 5.2 & 29.5 $\pm$ 6.2 & 4.4 $\pm$ 1.5 & 1.03 & 0.0\\
70.S12 & 13:01:58.1 & +29:32:08 & 3.9 & 3.4 $\pm$ 0.6 & 480 & 2.8 & 1.5 & 5.9 $\pm$ 6.1$^{\dagger}$ & 8.2 $\pm$ 5.6$^{\dagger}$ & 12.3 $\pm$ 6.0$^{\dagger}$ & 4.7 $\pm$ 1.6 & 1.05 & 0.1\\
70.S13 & 13:01:25.9 & +29:27:24 & 3.8 & 2.6 $\pm$ 0.5 & 430 & 2.5 & 1.3 & 8.4 $\pm$ 6.1$^{\dagger}$ & 17.6 $\pm$ 5.6$^{\dagger}$ & 29.3 $\pm$ 6.0$^{\dagger}$ & 4.2 $\pm$ 1.5 & 1.05 & 0.2\\
70.S14 & 13:01:39.4 & +29:32:28 & 3.7 & 0.7 $\pm$ 0.2 & 510 & 3.0 & 1.6 & 128.5 $\pm$ 6.2 & 76.3 $\pm$ 5.4 & 35.9 $\pm$ 5.7 & 5.0 $\pm$ 1.8 & 1.06 & 0.2\\
70.S15 & 13:01:55.0 & +29:32:08 & 3.7 & 2.4 $\pm$ 0.4 & 420 & 2.5 & 1.3 & 12.0 $\pm$ 6.1$^{\dagger}$ & 16.7 $\pm$ 5.6$^{\dagger}$ & 22.0 $\pm$ 6.0$^{\dagger}$ & 4.1 $\pm$ 1.5 & 1.06 & 0.2\\
70.S16 & 13:01:31.7 & +29:31:24 & 3.7 & 2.3 $\pm$ 0.4 & 370 & 2.2 & 1.1 & 16.5 $\pm$ 5.8 & 5.7 $\pm$ 5.8 & 3.6 $\pm$ 6.4 & 3.6 $\pm$ 1.3 & 1.06 & 0.2\\
70.S17 & 13:01:52.6 & +29:33:56 & 3.7 & 2.1 $\pm$ 0.4 & 630 & 3.7 & 1.9 & 21.2 $\pm$ 5.8 & 18.2 $\pm$ 5.7 & 8.8 $\pm$ 6.0 & 6.1 $\pm$ 2.2 & 1.06 & 0.3\\
70.S18 & 13:01:46.8 & +29:32:28 & 3.7 & 1.7 $\pm$ 0.4 & 400 & 2.3 & 1.2 & 23.4 $\pm$ 6.1$^{\dagger}$ & 17.2 $\pm$ 5.6$^{\dagger}$ & 10.1 $\pm$ 6.0$^{\dagger}$ & 3.9 $\pm$ 1.4 & 1.06 & 0.3\\
70.S19 & 13:01:22.0 & +29:26:28 & 3.6 & 1.5 $\pm$ 0.3 & 480 & 2.8 & 1.4 & 30.3 $\pm$ 6.0 & 20.4 $\pm$ 5.5 & 9.9 $\pm$ 6.0 & 4.6 $\pm$ 1.7 & 1.07 & 0.3\\
70.S20 & 13:02:03.0 & +29:30:16 & 3.5 & 1.6 $\pm$ 0.3 & 410 & 2.4 & 1.2 & 38.0 $\pm$ 5.8 & 31.3 $\pm$ 5.6 & 27.3 $\pm$ 5.7 & 4.0 $\pm$ 1.5 & 1.08 & 0.4\\
70.S21 & 13:01:37.3 & +29:31:12 & 3.5 & 1.9 $\pm$ 0.4 & 310 & 1.8 & 0.9 & 13.6 $\pm$ 5.6 & 16.5 $\pm$ 5.7 & 3.7 $\pm$ 5.9 & 3.0 $\pm$ 1.1 & 1.08 & 0.4\\
% 22 & 13:01:33.7 & +29:28:24 & 3.5 & 2.5 $\pm$ 0.5 & 313 & 1.8 & 0.9 & 12.0 $\pm$ 6.1$^{\dagger}$ & 5.5 $\pm$ 5.6$^{\dagger}$ & 14.6 $\pm$ 6.0$^{\dagger}$ & 3.0 $\pm$ 1.1 & 1.09 & 0.4\\
% 23 & 13:01:46 & +29:23:08 & 3.4 & 3.0 $\pm$ 0.5 & 570 & 3.3 & 1.7 & 13.5 $\pm$ 6.1$^{\dagger}$ & 10.0 $\pm$ 5.6$^{\dagger}$ & 14.3 $\pm$ 6.0$^{\dagger}$ & 5.4 $\pm$ 2.1 & 1.1 & 0.5\\
% 24 & 13:01:27 & +29:27:52 & 3.3 & 2.3 $\pm$ 0.4 & 373 & 2.2 & 1.1 & 13.2 $\pm$ 5.6 & 17.2 $\pm$ 5.8 & 30.9 $\pm$ 6.1 & 3.6 $\pm$ 1.4 & 1.11 & 0.5\\
% 25 & 13:01:20 & +29:30:48 & 3.3 & 2.4 $\pm$ 0.4 & 366 & 2.1 & 1.1 & 8.8 $\pm$ 6.1$^{\dagger}$ & 21.2 $\pm$ 5.6$^{\dagger}$ & 31.9 $\pm$ 6.0$^{\dagger}$ & 3.5 $\pm$ 1.4 & 1.11 & 0.5\\
% 26 & 13:01:56 & +29:25:44 & 3.3 & 2.4 $\pm$ 0.4 & 370 & 2.1 & 1.1 & 12.9 $\pm$ 6.1$^{\dagger}$ & 11.5 $\pm$ 5.6$^{\dagger}$ & 17.8 $\pm$ 6.0$^{\dagger}$ & 3.5 $\pm$ 1.4 & 1.11 & 0.5\\
% 27 & 13:01:43 & +29:24:48 & 3.3 & 2.4 $\pm$ 0.4 & 508 & 2.9 & 1.5 & 13.6 $\pm$ 6.1$^{\dagger}$ & 19.4 $\pm$ 5.6$^{\dagger}$ & 13.1 $\pm$ 6.0$^{\dagger}$ & 4.8 $\pm$ 1.9 & 1.11 & 0.5\\
% 28 & 13:01:48 & +29:28:36 & 3.3 & 2.8 $\pm$ 0.5 & 285 & 1.6 & 0.9 & 7.6 $\pm$ 6.1$^{\dagger}$ & 4.2 $\pm$ 5.6$^{\dagger}$ & 13.2 $\pm$ 6.0$^{\dagger}$ & 2.7 $\pm$ 1.1 & 1.12 & 0.6\\
% 29 & 13:01:46 & +29:25:28 & 3.2 & 4.6 $\pm$ 0.7 & 429 & 2.5 & 1.3 & 7.7 $\pm$ 6.1$^{\dagger}$ & 4.6 $\pm$ 5.6$^{\dagger}$ & -1.5 $\pm$ 6.0$^{\dagger}$ & 4.1 $\pm$ 1.6 & 1.12 & 0.6\\
% 30 & 13:01:41 & +29:25:12 & 3.2 & 3.1 $\pm$ 0.5 & 512 & 3.0 & 1.5 & 3.9 $\pm$ 6.1$^{\dagger}$ & 16.5 $\pm$ 5.6$^{\dagger}$ & 13.1 $\pm$ 6.0$^{\dagger}$ & 4.9 $\pm$ 1.9 & 1.12 & 0.6\\
% 31 & 13:01:27 & +29:29:00 & 3.2 & 2.7 $\pm$ 0.5 & 410 & 2.4 & 1.2 & 10.3 $\pm$ 6.1$^{\dagger}$ & 9.7 $\pm$ 5.6$^{\dagger}$ & 10.6 $\pm$ 6.0$^{\dagger}$ & 3.9 $\pm$ 1.6 & 1.12 & 0.6\\
% 32 & 13:01:29 & +29:27:24 & 3.2 & 1.6 $\pm$ 0.3 & 304 & 1.8 & 0.9 & 22.2 $\pm$ 5.8 & 24.9 $\pm$ 5.4 & 15.1 $\pm$ 6.0 & 2.9 $\pm$ 1.2 & 1.13 & 0.6\\
% 33 & 13:01:31 & +29:25:12 & 3.2 & 2.0 $\pm$ 0.4 & 369 & 2.1 & 1.1 & 16.3 $\pm$ 5.5 & 11.4 $\pm$ 5.7 & 4.6 $\pm$ 6.2 & 3.5 $\pm$ 1.4 & 1.13 & 0.6\\
% 34 & 13:01:34 & +29:24:36 & 3.2 & 2.9 $\pm$ 0.5 & 410 & 2.4 & 1.2 & 7.9 $\pm$ 6.1$^{\dagger}$ & 10.9 $\pm$ 5.6$^{\dagger}$ & 9.7 $\pm$ 6.0$^{\dagger}$ & 3.9 $\pm$ 1.6 & 1.13 & 0.6\\
% 35 & 13:01:58 & +29:33:16 & 3.1 & 2.7 $\pm$ 0.5 & 530 & 3.1 & 1.6 & 14.1 $\pm$ 6.1$^{\dagger}$ & 11.2 $\pm$ 5.6$^{\dagger}$ & 7.7 $\pm$ 6.0$^{\dagger}$ & 5.1 $\pm$ 2.0 & 1.13 & 0.6\\
% 36 & 13:01:35 & +29:30:00 & 3.1 & 2.1 $\pm$ 0.4 & 250 & 1.4 & 0.7 & 7.3 $\pm$ 6.1$^{\dagger}$ & 14.6 $\pm$ 5.6$^{\dagger}$ & 7.0 $\pm$ 6.0$^{\dagger}$ & 2.4 $\pm$ 1.0 & 1.13 & 0.6\\
% 37 & 13:01:56 & +29:28:12 & 3.1 & 2.4 $\pm$ 0.4 & 309 & 1.8 & 0.9 & 10.9 $\pm$ 6.1$^{\dagger}$ & 9.9 $\pm$ 5.6$^{\dagger}$ & 18.1 $\pm$ 6.0$^{\dagger}$ & 3.0 $\pm$ 1.2 & 1.15 & 0.7\\
% 38 & 13:01:40 & +29:35:44 & 3.1 & 6.0 $\pm$ 0.9 & 628 & 3.6 & 1.9 & 6.8 $\pm$ 6.1$^{\dagger}$ & 0.9 $\pm$ 5.6$^{\dagger}$ & 4.6 $\pm$ 6.0$^{\dagger}$ & 6.0 $\pm$ 2.5 & 1.15 & 0.7\\
% 39 & 13:01:29 & +29:34:12 & 3.1 & 2.2 $\pm$ 0.4 & 472 & 2.7 & 1.4 & 20.4 $\pm$ 6.0 & 31.1 $\pm$ 5.7 & 29.8 $\pm$ 6.5 & 4.5 $\pm$ 1.9 & 1.15 & 0.7\\
% 40 & 13:01:35 & +29:30:20 & 3.0 & 2.1 $\pm$ 0.4 & 247 & 1.4 & 0.7 & 7.3 $\pm$ 6.1$^{\dagger}$ & 14.6 $\pm$ 5.6$^{\dagger}$ & 12.2 $\pm$ 6.0$^{\dagger}$ & 2.4 $\pm$ 1.0 & 1.15 & 0.7\\
% 41 & 13:02:04 & +29:26:08 & 3.0 & 1.4 $\pm$ 0.3 & 499 & 2.9 & 1.5 & 22.5 $\pm$ 5.6 & 14.0 $\pm$ 5.6 & 4.1 $\pm$ 5.5 & 4.8 $\pm$ 2.0 & 1.15 & 0.7\\
% 42 & 13:01:58 & +29:35:28 & 3.0 & 5.7 $\pm$ 0.9 & 2997 & 17.3 & 9.0 & 10.7 $\pm$ 6.1$^{\dagger}$ & 16.5 $\pm$ 5.6$^{\dagger}$ & 24.2 $\pm$ 6.0$^{\dagger}$ & 28.6 $\pm$ 11.9 & 1.15 & 0.7\\
% 43 & 13:01:55 & +29:26:28 & 3.0 & 2.7 $\pm$ 0.5 & 282 & 1.6 & 0.8 & 13.2 $\pm$ 6.1$^{\dagger}$ & 1.6 $\pm$ 5.6$^{\dagger}$ & 2.5 $\pm$ 6.0$^{\dagger}$ & 2.7 $\pm$ 1.1 & 1.16 & 0.7\\
% 44 & 13:01:34 & +29:36:04 & 3.0 & -0.5 $\pm$ 0.1 & 813 & 4.7 & 2.4 & 22.3 $\pm$ 6.1$^{\dagger}$ & 4.1 $\pm$ 5.6$^{\dagger}$ & 3.5 $\pm$ 6.0$^{\dagger}$ & 7.8 $\pm$ 3.2 & 1.16 & 0.8\\
    \hline \end{tabular}
\raggedright \justify \vspace{-0.2cm}
\textbf{Notes:} 
Col. 1: The source identification of the sources shown in Figure~\ref{fig:mapOfHerBS70}. 
Col. 2 \& 3: The right ascension and declination of the sources.
Col. 4: The signal-to-noise ratio of the sources from the map, extracted from the peak pixel using the raw signal and noise of the sources, i.e., uncorrected for Eddington bias that is included in column 12.
Col. 5: Photometric redshift derived using the two-temperature modified black-body from \cite{pearson13}. 
Col. 6: The bolometric infrared luminosity ($8-1000$\micron{}), derived from the deboosted 850$\mu$m flux density assuming $z = 2.3$. We assume a single-temperature modified black-body at 30~K.
Col. 7: The star-formation rate derived from the FIR luminosity-to-SFR conversion factor, $1.73 \times 10^{-10}\ \mathrm{M_{\odot} yr^{-1}/L_{\odot}}$, is valid for a Salpeter $1-100\ \mathrm{M_{\odot}}$ IMF \citep{kennicutt1998}.
Col. 8: The dust mass estimate assuming a single-temperature modified black-body at 30~K at $z = 2.3$, assuming $\kappa_{d} = 10.41$~cm$^2$/g at 1900~GHz, and scaling according to $\kappa_{d}(\nu/\nu_{\rm ref})^{\beta}$ with $\beta = 2$ following \cite{draine2003}.
Col. 9, 10 \& 11: The {\it Herschel} photometry derived from the HELP catalogue. When unavailable (indicated by a \,$^{\dagger}$), we extract the fluxes directly from the {\it Herschel} maps (\url{www.h-atlas.org}) and use the errors documented in \cite{valiante2016}. 
Col. 12: The 850~\micron{} fluxes and errors, corrected for flux boosting, with the errors including both the instrumental and observational biases.
Col. 13: The flux boosting bias.
Col. 14: The false-positive probability, as a probability between 0 and 1.
\end{table*}
% \end{adjustbox}

}

% \end{landscape}

